FCoReBench: Can Large Language Models Solve Challenging First-Order Combinatorial Reasoning Problems?

Can the large language models (LLMs) solve challenging first-order combinatorial reasoning problems such as graph coloring, knapsack, and cryptarithmetic? By first-order, we mean these problems can be instantiated with potentially an infinite number of problem instances of varying sizes. They are also challenging being NP-hard and requiring several reasoning steps to reach a solution. While existing work has focused on coming up with datasets with hard benchmarks, there is limited work which exploits the first-order nature of the problem structure. To address this challenge, we present FCoReBench, a dataset of 40 such challenging problems, along with scripts to generate problem instances of varying sizes and automatically verify and generate their solutions. We first observe that LLMs, even when aided by symbolic solvers, perform rather poorly on our dataset, being unable to leverage the underlying structure of these problems. We specifically observe a drop in performance with increasing problem size. In response, we propose a new approach, SymPro-LM, which combines LLMs with both symbolic solvers and program interpreters, along with feedback from a few solved examples, to achieve huge performance gains. Our proposed approach is robust to changes in the problem size, and has the unique characteristic of not requiring any LLM call during inference time, unlike earlier approaches. As an additional experiment, we also demonstrate SymPro-LM's effectiveness on other logical reasoning benchmarks.

==> sections/abstract.tex <==
%Recent works show that the largest of the large language models (LLMs) can solve many simple reasoning tasks expressed in natural language, without any/much supervision. But, 

Can the largest large language models (LLMs) solve challenging first-order combinatorial reasoning problems such as graph coloring, knapsack, and cryptarithmetic? These problems are first-order, meaning they can be instantiated with any number of problem instances of varying sizes. They are also challenging being NP-hard and requiring several reasoning steps to reach a solution. To answer this question, we present \OurDatasetName{}, a dataset of $\NUMPUZZLESPUZZLEBENCH$ such challenging problems, along with scripts to generate problem instances and verify/generate their solutions. We first observe that LLMs, even when aided by symbolic solvers, perform rather poorly on our dataset, being unable to leverage the underlying structure of these problems. In response, we propose a new approach, \OurMethodName{}, which combines LLMs with both symbolic solvers and program interpreters, along with feedback from a few solved examples, to achieve huge performance gains. We also demonstrate \OurMethodName{}'s effectiveness 
%of integrating LLMs with symbolic solvers through programs 
on other logical reasoning benchmarks. Our extensive experimentation and analyses offer new insights into the reasoning abilities and limitations of present-day LLMs.

==> sections/abstract_neurips.tex <==
%Recent works show that the largest of the large language models (LLMs) can solve many simple reasoning tasks expressed in natural language, without any/much supervision. But, 

Can largest of the large language models (LLMs) solve challenging first-order combinatorial reasoning problems, such as graph coloring, knapsack and cryptarithmetic? 
To answer this question, we present \OurDatasetName{}, a dataset of $\NUMPUZZLESPUZZLEBENCH$ such challenging problems, along with a few solved instances for each problem. These problems are all first order, i.e., they can be instantiated with problem instances of varying sizes, and most of them are NP-hard, requiring several reasoning steps to reach the solution. 
We first observe that LLMs, even when aided by symbolic solvers, perform rather poorly on our dataset. In response, we propose a new approach, \OurMethodName{}, which combines LLMs with both symbolic solvers and program interpreters, along with feedback from solved examples, to achieve huge performance gains. We also demonstrate \OurMethodName{}'s effectiveness 
%of integrating LLMs with symbolic solvers through programs 
on other logical reasoning benchmarks. Our extensive experimentation and analyses offer new insights into the reasoning abilities and limitations of present-day LLMs.

==> sections/acknowledgments.tex <==
Mausam is supported by grants from Google, Huawei, and Jai Gupta Chair Professorship from IIT Delhi. Parag was supported by the DARPA Explainable Artificial Intelligence (XAI) Program (\#N66001-17-2-4032). Mausam and Parag are also supported by IBM SUR awards. Any opinions, findings, conclusions, or recommendations expressed here are those of the authors and do not necessarily reflect the views or official policies, either expressed or implied, of the funding agencies. We also acknowledge the Microsoft Accelerate Foundation Models Research Program for GPT4 access

==> sections/checklists.tex <==
% \begin{enumerate}

% \item {\bf Claims}
%     \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The abstract and introduction include the main claims/results of the paper and these are justified in the results section.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
%         \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
%         \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
%         \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
%     \end{itemize}

% \item {\bf Limitations}
%     \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The conclusion and limitations section which discusses the limitations of our work.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
%         \item The authors are encouraged to create a separate "Limitations" section in their paper.
%         \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
%         \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
%         \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
%         \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
%         \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
%         \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
%     \end{itemize}

% \item {\bf Theory Assumptions and Proofs}
%     \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: There are no theoretical results in our paper.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include theoretical results. 
%         \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
%         \item All assumptions should be clearly stated or referenced in the statement of any theorems.
%         \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
%         \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
%         \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
%     \end{itemize}

%     \item {\bf Experimental Result Reproducibility}
%     \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
%     \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The Experimental setup and the Appendix detail prompts/parameter setting used for our experiments which can be used to reproduce the results. We also release the dataset and the code.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
%         \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
%         \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
%         \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
%         \begin{enumerate}
%             \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
%             \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
%             \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
%             \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
%         \end{enumerate}
%     \end{itemize}


% \item {\bf Open access to data and code}
%     \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
%     \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: We release the dataset and code used in our experiments.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that paper does not include experiments requiring code.
%         \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
%         \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
%         \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
%         \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
%         \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
%         \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
%     \end{itemize}


% \item {\bf Experimental Setting/Details}
%     \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
%     \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The experiments setup section and appendix contain all details for settings used for our experiments. 
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
%         \item The full details can be provided either with the code, in appendix, or as supplemental material.
%     \end{itemize}

% \item {\bf Experiment Statistical Significance}
%     \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: For the main claims made by the paper, we perform significance tests via bootstrap resampling, and all improvements of our method over the baselines are statistically significant (p < 0.05).
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
%         \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
%         \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
%         \item The assumptions made should be given (e.g., Normally distributed errors).
%         \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
%         \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
%         \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
%         \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
%     \end{itemize}

% \item {\bf Experiments Compute Resources}
%     \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our experiments were primarily done through APIs but appendix~\ref{sec:appendix-experimental-details} contains details regarding this.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not include experiments.
%         \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
%         \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
%         \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
%     \end{itemize}
    
% \item {\bf Code Of Ethics}
%     \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The research conforms to the NeurIPS ethics code.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
%         \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
%         \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
%     \end{itemize}


% \item {\bf Broader Impacts}
%     \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
%     \item[] Answer: \answerNA{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our paper is on fundamental research and not tied to any particular application and we do not believe there is a direct societal impact of the work performed.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that there is no societal impact of the work performed.
%         \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
%         \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
%         \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
%         \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
%         \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
%     \end{itemize}
    
% \item {\bf Safeguards}
%     \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our paper does not have any such risks.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper poses no such risks.
%         \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
%         \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
%         \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
%     \end{itemize}

% \item {\bf Licenses for existing assets}
%     \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Problems in our dataset have existed for a long time some problem names are licensed but we create our own instances/rules which are not subject to copyright/licensing.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not use existing assets.
%         \item The authors should cite the original paper that produced the code package or dataset.
%         \item The authors should state which version of the asset is used and, if possible, include a URL.
%         \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
%         \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
%         \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
%         \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
%         \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
%     \end{itemize}

% \item {\bf New Assets}
%     \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
%     \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The released dataset is well documented.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not release new assets.
%         \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
%         \item The paper should discuss whether and how consent was obtained from people whose asset is used.
%         \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
%     \end{itemize}

% \item {\bf Crowdsourcing and Research with Human Subjects}
%     \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: Our paper does not involve any crowdsourcing or researching with human subjects.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
%         \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
%     \end{itemize}

% \item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
%     \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
%     \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
%     \item[] Guidelines:
%     \begin{itemize}
%         \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
%         \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
%         \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
%         \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
%     \end{itemize}

% \end{enumerate}

==> sections/conclusion.tex <==
We investigate the reasoning abilities of LLMs on structured first-order combinatorial reasoning problems. We formally define the task, and we present \texttt{\OurDatasetName}, a novel benchmark of $\NUMPUZZLESPUZZLEBENCH$ such problems and find that existing tool-augmented techniques, such as Logic-LM and PAL fare poorly. In particular, Logic-LM struggles with leveraging the structure of \fcore{} problems due to its inherent inability to handle implicit loops and conditionals.  Code interpreters manage loops and conditionals effectively, but directly writing reasoning code leads to incorrect programs.
Symbolic solvers excel in reasoning but require specific language formulations. 
Combining all these tools optimally, we propose \texttt{\OurMethodName} -- a new technique to aid LLMs with both program interpreters and symbolic solvers.
It uses LLMs to convert text into executable code, which is then processed by interpreters to define constraints, allowing symbolic solvers to efficiently tackle the reasoning tasks. Our extensive experiments show that \OurMethodName{}'s integrated approach leads to superior performance on our dataset as well as existing benchmarks. We also show that LLMs can write size-invariant code and find that they can use small sized solved examples to automatically debug their code. Further error analysis reveals that $\texttt{\OurMethodName}$ struggles for a certain class of problems where conversion to symbolic representation is not straightforward. In such cases simple feedback strategies do not improve reasoning; exploring methods to alleviate such problems is a promising direction for future work. Another future work direction is to extend this dataset to include images of inputs and outputs, instead of serialized text representations, and assess the reasoning abilities of vision-language models, like GPT4-V. 

\textbf{Limitations:} Adding new problems to \OurDatasetName{} requires reasonable manual effort in terms of writing the natural language rules and accompanying scripts. While we study a wide variety of \fcore{} problems, more such problems always exist and adding these to \OurDatasetName{} remains a direction of future work. Additionally we assume that input instances and their outputs have a fixed pre-defined (serialized) representation, which may not always be easy to find. Very large language models like GPT-4 have been trained on extremely large web corpora. While we write rules in our own words and generate instances synthetically, it is hard to know the extent of contamination. Encoding of many problems in the solver's language can potentially be complicated. Our method relies on the pre-training of LLMs to achieve this without any training/fine-tuning. 

==> sections/ethics.tex <==
\citep{StrubellGM19} show that the financial and environmental costs that are associated with the training of LLMs lead to significant contribution to global warming. We don't train the model from scratch and leverage in context learning, so the energy footprint of our work is less. The large language models whose API we use for inference, especially GPT-4, consume significant energy.

==> sections/introduction.tex <==

Recent works have shown that large language models (LLMs) can reason like humans \citep{DBLP:journals/tmlr/WeiTBRZBYBZMCHVLDF22}, and solve diverse natural language reasoning tasks, without the need for any fine-tuning \citep{wei2022chain, ZhouSHWS0SCBLC23, abs-2304-09797}. We note that, while impressive, these tasks are simple reasoning problems, generally requiring only a handful of reasoning steps to reach a solution.

We are motivated by the goal of assessing the reasoning limits of modern-day LLMs. In this paper, we study computationally intensive, first-order combinatorial problems posed in natural language. 
These problems (e.g., sudoku, knapsack, graph coloring, cryptarithmetic) have long served as important testbeds to assess the intelligence of AI systems \citep{russel2010}, and strong traditional AI methods have been developed for them. Can LLMs solve these directly? If not, can they solve these with the help of symbolic AI systems like SMT solvers?
To answer these questions, we release a dataset named \OurDatasetName{}, consisting of $\NUMPUZZLESPUZZLEBENCH$ such problems (see Figure~\ref{fig:puzzle-bench}). 

We refer to such problems as \emph{fcore} (\underline{f}irst-order \underline{co}mbinatorial \underline{re}asoning) problems. \emph{Fcore} problems can be instantiated with any number of instances of varying sizes, e.g., 9$\times$9 and 16$\times$16 sudoku. Most of the problems in  \OurDatasetName{} are NP-hard and solving them will require extensive planning and search over a large number of combinations. We provide scripts to generate instances for each problem and verify/generate their solutions. Across all problems we generate \NUMTESTINSTANCES{} test instances of varying sizes for evaluation and also provide \NUMTRAININSTANCES{} smaller sized solved instances as a training set. 

Not surprisingly, our initial experiments reveal that even the largest LLMs can only solve less than a third of these instances.
We then turn to recent approaches that augment LLMs with tools for better reasoning.  Program-aided Language models (PAL) \citep{gao2023pal} use LLMs to generate programs, offloading execution to a program interpreter. 
Logic-LM \citep{DBLP:conf/emnlp/PanAWW23} and SAT-LM \citep{Ye-Et-Al:2023:SAT} use LLMs to convert questions to symbolic representations, and external symbolic solvers perform the actual reasoning. 
Our experiments show that, by themselves, their performances are not that strong on \OurDatasetName{}.
At the same time, both these methods demonstrate complementary strengths -- PAL can handle first-order structures well, whereas Logic-LM is better at complex reasoning. 
In response, we propose a new approach named \OurMethodName{}, which combines the powers of \emph{both} PAL and symbolic solvers with LLMs to effectively solve \fcore{} problems. In particular, the LLM  generates an instance-agnostic program for an \fcore{} problem that converts any problem instance to a symbolic representation. This program passes this representation to a symbolic solver, which returns a solution back to the program. The program then converts the symbolic solution to the desired output representation, as per the natural language instruction. Interestingly, in contrast to LLMs with symbolic solvers, once this program is generated, inference on new \fcore{} instances (of any size) can be done \emph{without} any LLM calls.

\OurMethodName{} outperforms few-shot prompting by $21.61$, PAL by $3.52$ and Logic-LM by $16.83$ percent points on \texttt{\OurDatasetName}, with GPT-4-Turbo as the LLM. Given the structured nature of \fcore{} problems,  we find that utilizing feedback from small sized solved examples to correct the programs generated for just four rounds yields a further $21.02$ percent points gain for \OurMethodName{}, compared to $12.5$ points for PAL. 

We further evaluate \OurMethodName{} on three (non-first order) logical reasoning benchmarks from literature \citep{TafjordDC21, srivastava2023beyond, DBLP:conf/iclr/Saparov023}. \OurMethodName{} consistently outperforms existing baselines by large margins on two datasets, and is competitive on the third, underscoring the value of integrating LLMs with symbolic solvers through programs. We perform additional analyses to understand impact of hyperparameters on \OurMethodName{} and its errors.  We release the dataset and code for further research. We summarize our contributions below:
\begin{itemize}
    \item We formally define the task of natural language first-order combinatorial reasoning and present \OurDatasetName{}, a corresponding benchmark.
    \item We provide a thorough evaluation of LLM prompting techniques for \fcore{} problems, offering new insights into existing techniques.
    \item We propose a novel approach, \OurMethodName{}, demonstrating its effectiveness on \fcore{} problems as well as other datasets, along with an in-depth analysis of its performance.
\end{itemize}

% more lines here on insight if possible


\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{Images/puzzle-bench.png}
\caption{Illustrative examples of problems in \OurDatasetName{} (represented as images for illustration).}

  \label{fig:puzzle-bench}
\end{figure}

==> sections/introduction_neurips.tex <==

Recent works have shown that large language models (LLMs) can reason like humans \citep{DBLP:journals/tmlr/WeiTBRZBYBZMCHVLDF22}, and solve diverse natural language reasoning tasks, without the need for any fine-tuning \citep{wei2022chain, ZhouSHWS0SCBLC23, abs-2304-09797}. We note that, while impressive, these tasks are simple reasoning problems, generally requiring only a handful of reasoning steps to reach a solution.

We are motivated by the goal of assessing the reasoning limits of modern-day LLMs. In this paper, we study the computationally intensive, first-order combinatorial problems posed in natural language. 
These problems (e.g., sudoku, knapsack, graph coloring, cryptarithmetic) have long served as important testbeds to assess the intelligence of AI systems \citep{russel2010}, and strong traditional AI methods have been developed for them. Can LLMs solve these directly? If not, can they solve these with the help of symbolic AI systems like SMT solvers?
To answer these questions, we release a dataset named \OurDatasetName{}, consisting of $\NUMPUZZLESPUZZLEBENCH$ such problems along with a few solved instances of each problem (see Figure~\ref{fig:puzzle-bench}). 
We refer to such problems as \emph{fcore} (\underline{f}irst-order \underline{co}mbinatorial \underline{re}asoning) problems. \emph{Fcore} problems can be instantiated with instances of varying sizes, e.g., 9$\times$9 and 16$\times$16 sudoku. Most of the problems in  \OurDatasetName{} are NP-hard and solving them will require extensive planning and search over a large number of combinations. Not surprisingly, our initial experiments reveal that even the largest LLMs can only solve less than a third of these problems.

We then turn to recent approaches that augment LLMs with tools for better reasoning.  Program-aided Language models (PAL) \citep{gao2023pal} use LLMs to generate programs, offloading execution to a program interpreter. 
Logic-LM \citep{DBLP:conf/emnlp/PanAWW23} and SAT-LM \citep{Ye-Et-Al:2023:SAT} use LLMs to convert questions to symbolic representations, and external symbolic solvers perform the actual reasoning. 
Our experiments show that, by themselves, their performances are not that strong on \OurDatasetName{}.
At the same time, both these methods demonstrate complementary strengths -- PAL can handle first-order structures well, whereas Logic-LM is better at complex reasoning. 
In response, we propose a new approach named \OurMethodName{}, which combines the powers of \emph{both} PAL and symbolic solvers with LLMs. In particular, the LLM  generates an instance-agnostic program for an \fcore{} problem that converts any problem instance to a symbolic representation. This program passes this representation to a symbolic solver, which returns a solution back to the program. The program then converts the symbolic solution to the desired output representation, as per the natural language instruction. Interestingly, in contrast to LLMs with symbolic solvers, once this program is generated, inference on new \fcore{} instances (of any size) can be done \emph{without} any LLM calls.

\OurMethodName{} outperforms few-shot prompting by $21.61$, PAL by $3.52$ and Logic-LM by $16.83$ percent points on \texttt{\OurDatasetName}, with GPT-4-Turbo as the LLM. Given the structured nature of \fcore{} problems, 
%we also show how solved examples of small sizes can help improve reasoning. 
we find that utilizing feedback from solved examples for just four rounds yields a further $21.02$ percent points gain for \OurMethodName{}, compared to $12.5$ points for PAL. 
%We perform additional analyses to understand the impact of other hyperparameters, and also describe the errors made by \OurMethodName{}. 
%While motivated by first-order reasoning, 
We further evaluate \OurMethodName{} on three (non-first order) logical reasoning benchmarks from literature \citep{TafjordDC21, srivastava2023beyond, DBLP:conf/iclr/Saparov023}. \OurMethodName{} consistently outperforms existing baselines by large margins on two datasets, and is competitive on the third, underscoring the value of integrating LLMs with symbolic solvers through programs. We perform additional analyses to understand impact of hyperparameters on \OurMethodName{} and its errors.  We release the dataset and code for further research.

% more lines here on insight if possible


\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{Images/puzzle-bench.png}
\caption{Illustrative examples of problems in \OurDatasetName{}.}

  \label{fig:puzzle-bench}
\end{figure}

==> sections/related.tex <==
\textbf{Neuro-Symbolic AI}: Our work falls in the broad category of neuro-symbolic AI \citep{DBLP:journals/nn/YuYLWP23} which builds models leveraging the complementary strengths of neural and symbolic methods. Several prior works build neuro-symbolic models for solving combinatorial reasoning problems \citep{PalmPW18, pmlr-v97-wang19e,  PaulusRMAM21, NandwaniJMS22, NandwaniRMS22}. These develop specialized problem-specific modules (that are typically not size-invariant), which are trained over large training datasets. In contrast, \OurMethodName{} uses LLMs, and bypasses problem-specific architectures, generalizes to problems of varying sizes, and is trained with very few solved instances.

\vspace{0.5ex}\noindent
\textbf{Reasoning with Language Models}: The previous paradigm to reasoning was fine-tuning of LLMs \citep{10.5555/3491440.3491977, TafjordDC21, yang-etal-2022-generating}, but as LLMs scaled, they have been found to reason well, when provided with in-context examples without any fine-tuning \citep{brown2020language, WeiTBRZBYBZMCHVLDF22}. Since then, many prompting approaches have been developed that leverage in-context learning. Prominent ones include Chain of Thought (CoT) prompting \citep{wei2022chain, KojimaGRMI22}, Least-to-Most prompting \citep{ZhouSHWS0SCBLC23}, Progressive-Hint prompting \citep{abs-2304-09797} and Tree-of-Thoughts (ToT) prompting \citep{corr/abs-2305-10601}. 
% These works generally study relatively simple reasoning tasks.

\vspace{0.5ex}\noindent
\textbf{Tool Augmented Language Models}: Augmenting LLMs with external tools has emerged as a way to solve complex reasoning problems \citep{DBLP:journals/corr/abs-2302-04761, corr/abs-2303-09014}. The idea is to offload a part of the task to specialized external tools, thereby reducing error rates. Program-aided Language models \citep{gao2023pal} invoke a Python interpreter over a program generated by an LLM. Logic-LM \citep{DBLP:conf/emnlp/PanAWW23} and SAT-LM \citep{Ye-Et-Al:2023:SAT} integrate reasoning of symbolic solvers with LLMs, which convert the natural language problem into a symbolic representation. \OurMethodName{} falls in this category and combines LLMs with \emph{both} program interpreters and symbolic solvers. 

% \vspace{0.5ex}\noindent
% \textbf{Answer Verification}: Several existing works verify the correctness of LLM's answers via an external validation, such as via symbolic solvers \citep{corr/abs-2301-01162}, or external databases \citep{corr/abs-2302-12813}. 
% In the same spirit, \OurMethodName{} utilizes solved examples in training set for verifying LLM's output, and provide feedback to LLMs, in case of errors.

\vspace{0.5ex}\noindent
\textbf{Logical Reasoning Benchmarks}: There are several reasoning benchmarks in literature, such as LogiQA \citep{LiuCLHWZ20} for mixed reasoning, GSM8K \citep{abs-2110-14168} for arithmetic reasoning, FOLIO \citep{abs-2209-00840} for first-order logic, PrOntoQA \citep{Saparov023} and ProofWriter \citep{TafjordDC21} for deductive reasoning, AR-LSAT \citep{abs-2104-06598} for analytical reasoning. These dataset are not first-order i.e. each problem is accompanied with a single instance (despite the rules potentially being described in first-order logic). We propose \OurDatasetName{}, which substantially extends the complexity of these benchmarks by investigating computationally hard, first-order combinatorial reasoning problems. Two recent works, NLGraph \citep{wang2023can} and NPHardEval \citep{fan2023nphardeval} study structured reasoning problems but they focus on exploring the reasoning ability of LLMs with respect to graph problems and through the lens of computationally complexity respectively. In contrast we study the more broader area of first-order reasoning and investigate the associated complexities of structured reasoning. They also study relatively few problems (only 8 and 10 respectively) and all NP-Hard problems in these datasets are also present in our benchmark.


%NPHardEval \citealp{fan2023nphardeval} is another concurrent work that explores the reasoning abilities of LLMs through the lens of computationally complexity. \OurDatasetName{} substantially extends the complexity of these benchmarks by investigating computationally hard first-order reasoning problems. We specifically note that none of these benchmarks look at first order reasoning problems, which is the main focus of this study.
%They study relatively few problems and all NP-Hard problems in NPHardEval are also present in our benchmark.



%\textbf{Logical Reasoning Benchmarks}: There are several reasoning benchmarks in literature, such as LogiQA \citep{LiuCLHWZ20} for mixed reasoning, GSM8K \citep{abs-2110-14168} for arithmetic reasoning, FOLIO \citep{abs-2209-00840} for first-order logic, PrOntoQA \citep{Saparov023} and ProofWriter \citep{TafjordDC21} for deductive reasoning, AR-LSAT \citep{abs-2104-06598} for analytical reasoning, and NLGraph \citep{wang2023can} for natural language graph problems. We propose \OurDatasetName{}, which substantially extends the complexity of these benchmarks by investigating computationally hard, first-order combinatorial reasoning problems. NPHardEval \citealp{fan2023nphardeval} is another concurrent work that explores the reasoning abilities of LLMs through the lens of computationally complexity. They study relatively few problems and all NP-Hard problems in NPHardEval are also present in our benchmark.

% and ReClor \citep{YuJDF20}

==> sections/results.tex <==
Table~\ref{tab:main-results} describes the main results for \texttt{\OurDatasetName}. Unsurprisingly, GPT-4-Turbo is hugely better than other LLMs. Mixtral 8x7B struggles on our benchmark indicating that smaller LLMs (even with mixture of experts) are not as effective at complex reasoning. Mixtral in general does badly, often doing worse than random (especially when used without refinement).
PAL and \texttt{\OurMethodName} tend to perform better than other baselines benefiting from the vast pre-training of LLMs on code \citep{DBLP:journals/corr/abs-2107-03374}. Logic-LM performs rather poorly with smaller LLMs indicating that they struggle to invoke symbolic solvers directly.

% We perform significance tests via bootstrap resampling, and all improvements of our method over the baselines are statistically significant (p < 0.05)

\begin{wraptable}{r}{0.65\textwidth}
\vspace{-5mm}
\captionsetup{font=small}
\caption{Results for \texttt{\OurDatasetName}. - / + indicate before / after \emph{refinement}. Performance for random guessing is 20.13\%.}
\label{tab:main-results}
\centering
\scalebox{0.65}{
\begin{tabular}{lccccccc}
\toprule
    & Few-Shot & \multicolumn{2}{c}{PAL} & \multicolumn{2}{c}{Logic-LM} & \multicolumn{2}{c}{\OurMethodName{}} \\
    Model & Prompting& - & + & - & + & - & + \\
    \midrule
    Mixtral 8x7B  & 25.06\% & 14.98\% & 36.09\% & 0.21\% & 2.04\% & 8.08\% & 30.09\% \\
    GPT-3.5-Turbo  & 27.02\% & 32.66\% & 49.19\% & 6.04\% & 6.58\% & 17.08\% & 50.35\%  \\
    GPT-4-Turbo  & 29.33\% & 47.42\% & 66.40\% & 34.11\% & 38.51\% & 50.94\% & \textbf{83.37\%} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{wraptable}

% random --> 20.13

%\textbf{\OurMethodName{} vs Baselines}: 
Hereafter, we focus primarily on GPT-4-Turbo’s performance, since it is far superior to other models. \texttt{\OurMethodName} outperforms few-shot prompting and Logic-LM across all problems in \texttt{\OurDatasetName}. On average the improvements are by an impressive $54.04\%$ against few-shot prompting and by $44.86\%$ against Logic-LM (with \emph{refinement}). Few-shot prompting solve less than a third of the problems with GPT-4-Turbo, suggesting that even the largest LLMs cannot directly perform complex reasoning. While Logic-LM performs better, it still isn't that good either, indicating that combining LLMs with symbolic solvers is not enough for such reasoning problems.

\begin{wraptable}{r}{0.42\textwidth} % "r" for right and "l" for left alignment
 \vspace{-8mm}\
\captionsetup{font=small}
\caption{Logic-LM's performance on \texttt{\OurDatasetName} evaluated with \emph{refinement}.}
\label{tab:logiclm-errors}
\centering
\scalebox{0.7}{
    \begin{tabular}{p{2.4cm} c c}
        \toprule
        \textbf{Outcome} & \textbf{GPT-3.5-Turbo} & \textbf{GPT-4-Turbo} \\
        \midrule
        Correct Output & 6.58\% & 38.51\% \\
        Incorrect Output & 62.11\% & 52.06\% \\
        Timeout Error & 2.375\% & 2.49\% \\
        Syntactic Error & 29.04\% & 6.91\% \\
        % Errors in Converting Symbolic Output to Text & 21.24\% & 12.34\% \\
        \bottomrule
    \end{tabular}
}
\vspace{-3mm}
\end{wraptable}

Further qualitative analysis suggests that Logic-LM gets confused in handling the structure of \fcore{} problems. As problem instance size grows, it tends to make syntactic mistakes with smaller LLMs (Table~\ref{tab:logiclm-errors}). With larger LLMs, syntactic mistakes reduce, but constraints still remain semantically incorrect and do not get corrected through feedback. Often this is because LLMs are error-prone when enumerating combinatorial constraints, i.e., they struggle with executing \emph{implicit} for-loops and conditionals (see Appendix~\ref{sec:appendix-logic-lm examples}). In contrast, \OurMethodName{} and PAL manage first order structures well, since writing code for a loop/conditional is not that hard, and the correct loop-execution is done by a program interpreter.
%instance-agnostic programs during training that can then be corrected through feedback from solved examples. 
%This showcases that LLMs can write size-invariant code and can perform debugging through feedback from a small number of solved examples. 
These (size-invariant) programs then get used independently without any LLM call at inference time to solve any input instance -- easily generalizing to larger instances --  highlighting the benefit of using a program interpreter for such combinatorial problems.


\begin{wraptable}{r}{0.48\textwidth}
\centering
\captionsetup{font=small}
\vspace{-5mm}
\caption{Error analysis at a program level for GPT-4-Turbo before and after \emph{refinement} for PAL and SymPro-LM. Results are averaged over all runs for a problem and further over all problems in \OurDatasetName{}.}
\label{tab:error-analysis}
\scalebox{0.64}{
\begin{tabular}{lcc}
\toprule
\textbf{Outcome} & \textbf{PAL} & \textbf{SymPro-LM} \\
& (Before / After) & (Before / After) \\
\midrule
Incorrect Program & 70\% / 57\% & 58\% / 38\% \\
Semantically Incorrect Program & 62\% / 49.5\% & 29\% / 20.5\% \\
Python Runtime Error & 7\% / 4.5\% & 13.5\% / 5.5\% \\
Timeout & 1\% / 3\% & 15.5\% / 12\% \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{wraptable}

At the same time, PAL is also not as effective on \OurDatasetName{}. 
Table~\ref{tab:pal-vs-puzzlelm} compares the effect of feedback and multiple runs on PAL and \texttt{\OurMethodName}. \texttt{\OurMethodName} outperforms PAL by $16.97\%$ on \texttt{\OurDatasetName} (with \emph{refinement}). 
When LLMs are forced to write programs for performing complicated reasoning, they tend to produce brute-force solutions that often are either incorrect or slow (see Table-\ref{tab:timing-comparison} in the appendix). 
This highlights the value of offloading  reasoning to a symbolic solver. Interestingly, feedback from solved examples and re-runs is more effective (Table ~\ref{tab:error-analysis})  for \texttt{\OurMethodName}, as also shown by larger gains with increasing number of feedback rounds and runs (Table ~\ref{tab:pal-vs-puzzlelm}). We hypothesize that this is because declarative programs (generated by \OurMethodName{}) are easier to correct, than imperative programs (produced by PAL).
%while PAL produces imperative programs which are more difficult to correct.


\begin{table}[h]
\vspace{-3mm}
\caption{Comparative analysis between PAL and \texttt{\OurMethodName} on \texttt{\OurDatasetName} for GPT-4-Turbo.}
\label{tab:pal-vs-puzzlelm}
\centering
\begin{subtable}[b]{0.49\textwidth}
    \centering
    \scalebox{0.65}{
    \begin{tabular}{c c c c c c}
        \toprule
        & \multicolumn{5}{c}{\textbf{Number of Rounds of Feedback}} \\
        \cmidrule{2-6}
        & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} \\
        \midrule
        \textbf{PAL} & 47.42\%  & 54.00\%  & 57.09\%  & 58.82\%  & 59.92\%  \\
        \textbf{\OurMethodName} & 50.94\%  & 62.54\%  & 68.52\%  & 71.12\%  & 71.96\%  \\
         & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{3.52\%}}
         & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{8.54\%}}
         & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{11.43\%}}
         & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{12.3\%}}
         & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{12.04\%}}\\
        \bottomrule
    \end{tabular}
    }
    \captionsetup{font=small}
    \caption{Effect of feedback rounds for a single run}
    \label{table:pal-vs-puzzlelm-feedback}
\end{subtable}%
\hfill
\begin{subtable}[b]{0.49\textwidth}
\centering
\scalebox{0.65}{
\begin{tabular}{c c c c c c}
\toprule
& \multicolumn{5}{c}{\textbf{Number of Runs}} \\
\cmidrule{2-6}
& \textbf{1} & \textbf{2} & \textbf{3}  & \textbf{4}  & \textbf{5}\\
\midrule
\textbf{PAL} & 59.92\% & 62.54\%  & 63.95\% & 65.19\% & 66.40\%  \\
\textbf{\OurMethodName} & 71.96\%  & 77.21\%  & 80.06\% & 82.06\% & 83.37\%   \\
 & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{12.04\%}}
 & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{14.67\%}}
 & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{16.11\%}}
 & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{16.87\%}}
 & \textcolor{OliveGreen}{$\uparrow$} \footnotesize{\textcolor{OliveGreen}{16.97\%}}\\
\bottomrule
\end{tabular}
}
\captionsetup{font=small}
\caption{Effect of multiple runs each with 4 feedback rounds}
\label{table:pal-vs-puzzlelm-restart}
\end{subtable}
\end{table}
\vspace{-3mm}


\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \vspace{-5mm}
    \captionsetup{font=small}
    \caption{Accuracy and cost comparison between ToT prompting and \texttt{\OurMethodName{}} with GPT-4-Turbo for 3 problems in \texttt{\OurDatasetName}. Costs are per test instance for ToT and one time costs per problem for \texttt{\OurMethodName{}}.}
    \label{tab:tot-results}
    \scalebox{0.70}{
    \begin{tabular}{llcccc}
        \toprule
        \multirow{2}{*}{Problem} & \multirow{2}{*}{Instance size} & \multicolumn{2}{c}{ToT prompting} & \multicolumn{2}{c}{\OurMethodName{}} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6}
         & & Accuracy & Cost & Accuracy & Cost \\
        \midrule
        \multirow{2}{*}{Latin Squares} 
         & 3x3 & 46.33\%& \$0.1235 & 100\% & \$0.02 \\
         & 4x4 & 32.5\%  & \$0.5135 & 100\% & \$0.02 \\
        \midrule
        \multirow{2}{*}{Magic Square} 
         & 3x3 & 26.25\% & \$0.4325  & 100\% & \$0.02 \\
         & 4x4 & 8\% & \$0.881 & 100\% & \$0.02 \\
        \midrule
        \multirow{2}{*}{Sujiko} 
         & 3x3 & 7.5\% & \$0.572 & 100\% & \$0.02 \\
         & 4x4 & 0\% & \$1.676 & 100\% & \$0.02 \\
        \bottomrule
    \end{tabular}}
    \vspace{-4mm}
\end{wraptable}

\textbf{Comparison with ToT Prompting}: Table~\ref{tab:tot-results} compares \OurMethodName{} with ToT prompting on 3 problems. \OurMethodName{} is far superior in terms of cost and accuracy, indicating that even the largest LLMs cannot do complex reasoning on problems with large search depths and branching factors, despite being called multiple times with search-based prompting. Due to its programmatic nature, \OurMethodName{} generalizes even better to larger instances and is also hugely cost effective, as there is no need to call an LLM for each instance separately. We do not perform further experiments with ToT prompting, due to cost considerations. 

% \begin{table}[h]
%     \centering
%     \vspace{-3mm}
%     \captionsetup{font=small}
%     \caption{Accuracy and cost comparison b/w ToT prompting and \texttt{\OurMethodName{}} for 3 problems in \texttt{\OurDatasetName}. Costs are per test instance for ToT and one time costs per problem for \texttt{\OurMethodName{}}.}
%     \label{tab:tot-results}
%     \scalebox{0.75}{
%     \begin{tabular}{llcccccccc}
%         \toprule
%         \multirow{2}{*}{Problem} & \multirow{2}{*}{Instance size} & \multicolumn{4}{c}{GPT-3.5-Turbo} & \multicolumn{4}{c}{GPT-4-Turbo} \\
%         \cmidrule(r){3-6} \cmidrule(r){7-10}
%          & & \multicolumn{2}{c}{ToT prompting} & \multicolumn{2}{c}{\OurMethodName{}} & \multicolumn{2}{c}{ToT prompting} & \multicolumn{2}{c}{\OurMethodName{}} \\
%          & & Accuracy & Cost & Accuracy & Cost & Accuracy & Cost & Accuracy & Cost \\
%         \midrule
%         \multirow{2}{*}{Latin Squares} 
%          & 3x3 & 11.67\% & \$0.0035 & 80\% & \$0.0024 & 46.33\%& \$0.1235 & 100\% & \$0.02 \\
%          & 4x4 & 6.25\% & \$0.0095 & 80\% & \$0.0024 & 32.5\%  & \$0.5135 & 100\% & \$0.02 \\
%         \midrule
%         \multirow{2}{*}{Magic Square} 
%          & 3x3 & 0\% & \$0.005 & 40\% &  \$0.005 & 26.25\% & \$0.4325  & 100\% & \$0.02 \\
%          & 4x4 & 0\% & \$0.003 & 40\% & \$0.005 & 8\% & \$0.881 & 100\% & \$0.02 \\
%         \midrule
%         \multirow{2}{*}{Sujiko} 
%          & 3x3 & 0\% & \$0.014 & 21\% & \$0.005 & 7.5\% & \$0.572 & 100\% & \$0.02 \\
%          & 4x4 & 0\% & \$0.0375 & 19\% & \$0.005 & 0\% & \$1.676 & 100\% & \$0.02 \\
%         \bottomrule
%     \end{tabular}}
% \end{table}



%\vspace{-3mm}
\begin{figure*}[htbp]
  \centering \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{Images/size-vs-algo.png}
  \captionsetup{font=small}
  \caption{Effect of increasing problem instance size on baselines and \OurMethodName{} for GPT-4-Turbo.}
  \label{fig:size-vs-algo}
\end{figure*}

\textbf{Effect of Problem Instance Size}: We now report performance of \OurMethodName{} and other baselines against varying problem instance sizes (see Figure~\ref{fig:size-vs-algo}) for 3 problems in \OurDatasetName{} (sudoku, sujiko and magic-square). Increasing the problem instance size increases the number of variables, accompanying constraints and reasoning steps required to reach the solution. We observe that being programmatic \OurMethodName{} and PAL, are relatively robust against increase in size of input instances. In comparison, performance of Logic-LM and few-shot prompting declines sharply. PAL programs are often inefficient and may see performance drop when they fail to find a solution within the time limit.



\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.325\textwidth} % 'b' for bottom alignment
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{Images/feedback-effect.png}
    \caption{Effect of feedback}
    \label{fig:effect-feedback}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
      \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{Images/effect-runs.png}
    \caption{Effect of multiple runs}
    \label{fig:effect-runs}
  \end{subfigure}
  \begin{subfigure}[b]{0.325\textwidth}
      \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{Images/solved-examples-count.png}
    \caption{Effect of \# of solved examples}
    \label{fig:number-of-examples}
  \end{subfigure}
  \captionsetup{font=small}
  \caption{Effect of feedback and multiple runs with GPT-4-Turbo. (a) and (b) show results with 10 solved examples for feedback where dashed lines show results for individual problems in \texttt{\OurDatasetName}, with coloured lines highlighting specific problems and the red bold line represents the average effect across all problems. (c) shows the effect of number of solved examples used for feedback in a single run.}
  \label{fig:re-runs-feedback-puzzle-lm-gpt-4}
\vspace{-4mm}
\end{figure*}


\textbf{Effect of Feedback on Solved Examples}: Figure~\ref{fig:effect-feedback} describes the effect of multiple rounds of feedback for \texttt{\OurMethodName}. Feedback helps performance significantly; utilizing 4 feedback rounds improves performance by $21.02\%$. Even the largest LLMs commit errors, making it important to verify and correct their work. But feedback on its own is not enough, a single run might end-up in a wrong reasoning path, which is not corrected by feedback making it important to utilize multiple runs for effective reasoning. Utilizing 5 runs improves the performance by additional $11.41\%$ (Figure~\ref{fig:effect-runs}) after which the gains tend to saturate. Performance also increases with an increase in the number of solved examples (Figure~\ref{fig:number-of-examples}). Each solved example helps in detecting and correcting different errors. However, performance tends to saturate at 7 solved examples and no new errors are discovered/corrected, even with additional training data.

\subsection{Results on Other Datasets}
\begin{table}[b]
\vspace{-6mm}
\captionsetup{font=small}
\caption{Results for baselines \& \OurMethodName{} on other benchmarks. Best results with each LLM are highlighted.} 
\label{tab:main-results-other-datasets}
\centering
\scalebox{0.7}{
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
& \multicolumn{5}{c}{GPT-3.5-Turbo-0125} & \multicolumn{5}{c}{GPT-4-Turbo-0125} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
Dataset & Direct & CoT & PAL & Logic-LM & \OurMethodName{} & Direct & CoT & PAL & Logic-LM & \OurMethodName{} \\ 
\midrule
Logical Deduction & 39.66 \% & 50.66 \% & 66.33 \% & 71.00 \% & \textbf{78.00 \%} & 65.33 \% & 76.00 \% & 81.66 \% & 82.67 \% & \textbf{94.00 \%} \\
ProofWriter & 40.50 \% & 57.16 \% & 50.5 \% & 70.16 \% & \textbf{74.167 \%} & 46.5 \% & 61.66 \% & 76.29 \% & 74.83 \% & \textbf{89.83 \%} \\
PrOntoQA & 49.60 \% & 83.20 \% & \textbf{98.40 \%} & 72.20 \% & 97.40 \% & 83.00 \% & 98.80 \% & \textbf{99.80 \%} & 91.20 \% & 97.80 \% \\
\bottomrule
\end{tabular}}
\end{table}

Table~\ref{tab:main-results-other-datasets} reports the performance on non-first order datasets. \OurMethodName{} outperforms all other baselines on ProofWriter and LogicalDeduction, particularly Logic-LM. This showcases the value of integrating LLMs with symbolic solvers through programs, even for standard reasoning tasks. These experiments suggest that LLMs translate natural language questions into programs using solvers much more effectively than into symbolic formulations directly. We attribute this to the vast pre-training of LLMs on code \citep{brown2020language,DBLP:journals/corr/abs-2107-03374}. For instance, on the LogicalDeduction benchmark, while Logic-LM does not make syntactic errors during translation it often makes logical errors. These errors significantly decrease when LLMs are prompted to produce programs instead (Figure~\ref{fig:logical-deduction-example}). Error analysis on ProofWriter and PrOntoQA reveals that for more complex natural language questions, LLMs also start making syntactic errors during translation as the number of rules/facts start increasing. With \OurMethodName{} these errors are vastly reduced because, apart from the benefit from pre-training, LLMs also start utilizing programming constructs like dictionaries and loops to make most out of the structure in these problems (Figure~\ref{fig:prontoqa-example}). PAL and CoT perform marginally better on PrOntoQA because the reasoning style for problems in this dataset involves forward-chain reasoning % i.e. beginning with known facts and sequentially deriving new conclusions until the goal is met 
which aligns with PAL's and CoT's style of reasoning. Integrating symbolic solvers is not as useful for this dataset, but still achieves competitive performance.



\begin{figure*}[h]
  \centering
  \begin{subfigure}[b]{0.5\textwidth} % 'b' for bottom alignment
    \adjustbox{valign=b}{\includegraphics[width=\textwidth]{Images/prontoQA-example.png}}
    \caption{PrOntoQA}
    \label{fig:prontoqa-example}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth} % 'b' for bottom alignment
    \adjustbox{valign=b}{\includegraphics[width=\textwidth]{Images/logicaldeduction-example.png}}
    \caption{LogicalDeduction}
    \label{fig:logical-deduction-example}
  \end{subfigure}
  \caption{Examples highlighting benefits of integrating LLMs with symbolic solver through programs.}
  \label{fig:other-dataset-examples}
\end{figure*}

